Top-Quark Physics Results From LHC

The top-quark is a fundamental element of the physics program at the Large Hadron Collider (LHC). We review the current status of the top-quark measurements performed by ATLAS and CMS experiments in pp collisions at sqrt(s)=7 TeV by presenting the recent results of the top-quark production rates, top mass measurements and additional top quark properties. We will also describe the recent searches for physics beyond the Standard Model in the top-quark sector.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips
BASENAME = LCWS11_fiorini
default: testlatex
testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	#bibtex ${BASENAME}
	#latex  ${BASENAME}
	#latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}
testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
#
# standard Latex targets
#
%.dvi:	%.tex 
	$(LATEX) $<
%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*
%.ps:	%.dvi
	$(DVIPS) $< -o $@
%.pdf:	%.tex
	$(PDFLATEX) $<
.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 
#

